Multi-modal Uncertainty Robust Tree Cover Segmentation For High-Resolution Remote Sensing Images

Recent advances in semantic segmentation of multi-modal remote sensing images have significantly improved the accuracy of tree cover mapping, supporting applications in urban planning, forest monitoring, and ecological assessment. Integrating data from multiple modalities-such as optical imagery, light detection and ranging (LiDAR), and synthetic aperture radar (SAR)-has shown superior performance over single-modality methods. However, these data are often acquired days or even months apart, during which various changes may occur, such as vegetation disturbances (e.g., logging, and wildfires) and variations in imaging quality. Such temporal misalignments introduce cross-modal uncertainty, especially in high-resolution imagery, which can severely degrade segmentation accuracy. To address this challenge, we propose MURTreeFormer, a novel multi-modal segmentation framework that mitigates and leverages aleatoric uncertainty for robust tree cover mapping. MURTreeFormer treats one modality as primary and others as auxiliary, explicitly modeling patch-level uncertainty in the auxiliary modalities via a probabilistic latent representation. Uncertain patches are identified and reconstructed from the primary modality's distribution through a VAE-based resampling mechanism, producing enhanced auxiliary features for fusion. In the decoder, a gradient magnitude attention (GMA) module and a lightweight refinement head (RH) are further integrated to guide attention toward tree-like structures and to preserve fine-grained spatial details. Extensive experiments on multi-modal datasets from Shanghai and Zurich demonstrate that MURTreeFormer significantly improves segmentation performance and effectively reduces the impact of temporally induced aleatoric uncertainty.

==> 6Acknowledgements.tex <==
This paper is supported by the National Key R\&D Program of China (Grant No.2021YFB390052).  We thank Melissa Dawes for professional language editing.

==> zh.tex <==
\begin{abstract}
\begin{CJK}{UTF8}{gbsn}
近年来，基于深度学习的多模态遥感图像语义分割技术获得飞速发展，其中tree cover类别的分割精度往往较高，这使得tree cover mapping作为一种可信度较高的信息常被用于城市规划、森林管理、ecosystem assessment等。除了常见的光学遥感图像、LiDAR,SAR等数据均有对tree cover观测的优势，将多模态用于mapping的精度往往高于单模态。然而在实际任务中，不同模态的遥感相机拍摄任务基本不是同一时间进行的，这导致同一区域的多模态遥感数据可能相差几天甚至几个月，而这对tree cover mapping有较高的干扰。短时间内发生的砍伐、火灾、台风等都能快速改变tree cover，而这种短时间内就会造成的差别将会影响多源数据像素或特征的融合，由于成本原因，这些错误往往作为uncertainty 原因被忽略。分辨率越高，这种uncertainty difference在遥感数据上就越明显。因此，为了充分的融合多模态特征并降低uncertainty带来的干扰，本工作设计了语义分割模型，称为MURTreeFormer(Multi-model uncertainty robust TreeFormer)。本任务将模态分为主模态与副模态，首先将多模态图像分为多个patch，并通过计算不同patch的分布来定位uncertainty patch，通过主模态的分布重建副模态，并充分融合。除此之外，网络基于pregressive decoder添加了针对tree cover 特征的grad magnitude attention 和tree edge aggregate block用于增强并恢复高分辨率的林地特征，进一步提高林地分割能力。网络不仅输出了tree cover mapping result，也输出了多模态数据间的uncertainty position，指出了可能的变化位置。我们在中国上海和瑞士苏黎世的多模态遥感数据集上进行了实验，结果表明，我们的模型可以充分融合不同模态的信息，提高林地的分类精度，且对可能的变化区域分辨正确率达到95%。
\end{CJK}
\end{abstract}

\begin{CJK}{UTF8}{gbsn}
多模态语义分割方法被广泛应用于行车场景分割\cite{li2022rgb,zhao2023mitigating}、医疗影像分割\cite{yang2022toward,sun2024semi}等任务中。近几年，基于深度学习的multi-modal fusion encoder已经可以在不同任务中充分融合不同的模态特征，添加适当的decoder后，即可形成完整的网络进行分割任务。\citet{jia2024geminifusion} proposed GeminiFusion, a linear-complexity pixel-wise fusion framework that harmonizes intra- and inter-modal attention through layer-adaptive noise control for efficient cross-modal integration. \citet{wan2025sigma} proposed Sigma, a Siamese Mamba network for efficient multi-modal segmentation that achieves global receptive fields with linear complexity through a novel Mamba-based fusion mechanism and enhanced channel-wise decoding. 这些任务中的多模态数据往往来自于同一时相，因此对于uncertainty多是讨论section2.1中如何balance
the learning contributions of different modalitie。

在遥感地物识别方面，近些年有许多优秀的多模态语义分割模型被提出。 TransFusion enables direct image-point cloud fusion for semantic segmentation without lossy pre-processing, effectively learning spatial and structural information for improved inference \cite{maiti2023transfusion}. \citet{zhang2024asanet} propose the Asymmetric Semantic Aligning Network (ASANet), which introduces asymmetry at the feature level to address the issue that multi-modal architectures frequently fail to fully utilize complementary features. \citet{li2022mcanet} proposed the MCANet, which is a multimodal-cross attention network featuring a pseudo-siamese encoder for ORS and SAR feature extraction, second-order hidden feature mining via cross-modal attention, and multi-scale feature fusion. 这些遥感任务基本使用了公开数据集，因此并不需要考虑uncertainty为分割精度带来的影响，而实际问题中，出于成本考虑，uncertainty也往往被直接忽略。此外，这些模型并非针对tree cover，在高分辨率图像中tree cover的细节分割结果未达到最佳。
\end{CJK}

\section{Methodology}
\begin{CJK}{UTF8}{gbsn}
在patch embedding后，主模态与副模态被分割成不重叠的patches，形成n组patch。
To a large extent, the variance reflects the dispersion of the distribution. When the landcover undergoes temporal changes, the corresponding image patch deviates from its neighbors and its latent distributional feature demonstrates dispersive behavior. As thus, we propose to use the determinant of co-variance matrix, \textit{i.e.,} $\Big\vert\mathsf{diag}(\mathbf{\sigma}_M^{(i)})\Big\vert=\prod_{i=1}^d\mathbf{\sigma}_M^{(i)}[i]$, to measure the dispersion extent of the distributional representation. Then the ratio, $\frac{\Big\vert\mathsf{diag}(\mathbf{\sigma}_O^{(i)})\Big\vert}{\Big\vert\mathsf{diag}(\mathbf{\sigma}_A^{(i)})\Big\vert}$, measures the distributional inconsistency of the two modalities, which is employed as the criterion for us to identify the unmatched patches from $\mathcal{X}_A$. However, to avoid overflow, we further improve to use $\log\left(\frac{\Big\vert\mathsf{diag}(\mathbf{\sigma}_O^{(i)})\Big\vert}{\Big\vert\mathsf{diag}(\mathbf{\sigma}_A^{(i)})\Big\vert}\right)$, which is equivalent to the entropy difference:
\begin{equation}
	\begin{aligned}
		\mathsf{ED}&\left(\mathsf{p}\left(\mathbf{z}_O^{(i)}|\mathbf{x}_O^{(i)}\right),\mathsf{p}\left(\mathbf{z}_A^{(i)}|\mathbf{x}_A^{(i)}\right)\right)\triangleq\\&\mathsf{H}\left(\mathsf{p}\left(\mathbf{z}_O^{(i)}|\mathbf{x}_O^{(i)}\right)\right)-\mathsf{H}\left(\mathsf{p}\left(\mathbf{z}_A^{(i)}|\mathbf{x}_A^{(i)}\right)\right)
	\end{aligned}
\end{equation}
where $\mathsf{H}\left(\mathsf{p}\left(\cdot\right)\right)$ calculates the entropy of some distribution $\mathsf{p}\left(\cdot\right)$. Then we sort out a $K$-element set $\mathbb{T}\subset\left\{1,2,\cdots,N\right\}$ such that
\begin{equation}
	\begin{aligned}
    &\mathbb{T}=\\&\underset{_{\vert\mathbb{T}\vert=K}}{\arg\max}(\min(\Big\{\Big\vert\mathsf{ED}\left(\mathsf{p}\left(\mathbf{z}_O^{(t)}|\mathbf{x}_O^{(t)}\right),\mathsf{p}\left(\mathbf{z}_A^{(t)}|\mathbf{x}_A^{(t)}\right)\right)\Big\vert\Big\}_{t\in\mathbb{T}})).
	\end{aligned}
\end{equation}
Thereupon, $\mathbb{T}$ indexes $K$ patches with the largest absolute entropy difference value from the auxiliary modality as the ones needs reconstruction.


如前文所说，多模态不确定性的重新建立已有相关研究，但基于语义分割的多模态重建研究是空白的。这是因为多模态任务将图片作为整体直接编码，可是语义分割任务若以像素级编码将产生巨大的计算量，因此，本研究创新地按patch级进行uncertainty检测与重建。To balance the computational burden and granularity of data processing, SURM firstly divides each modality $\mathcal{X}_M,\,M\in\left\{O,A\right\}$ into non-overlapping patches $\mathcal{X}_M^{(i)},\,i=1,2,\cdots,N.$ Then SURM learns the parametric distributional representations of the latent features from the initial embedding of those patches, $\mathbf{x}_M^{(i)}\in\mathbb{R}^D$. Based on the distributional parameters, SURM locates the untrustworthy patch embeddings in the auxiliary modality.而将uncertainty结果输出，即可视为两个多模态图像输入的uncertainty postions，MURTreeFormer的patch大小为 4\times4，因此，如图所示，可视化效果较好。

基于vae的重建原理是按照目标分布随机生成大量的token，从而拟合出目标分布，这显然会产生巨量的计算，因此在像素级计算机视觉任务上未被应用过。SURM创新性地使用uncertainty patch来引导重建任务。 reconstruct their features according to the corresponding features of the primary modality. After distribution alignment, those features will be weighting-integrated according to their distributional parameters in the CDFM. 

具体来说，Drawing inspiration from Multi-modal fusion \cite{bibid}, we learn parametric distributions from the patch embeddings to achieve fuzzy feature representation that is capable of uncertainty modeling. To this end, we assign a mutual-independent multi-variate Gaussian distribution to its latent feature representation $\mathbf{z}_M^{(i)}\in\mathbb{R}^d$ conditioned on $\mathbf{x}_M^{(i)}$, \textit{i.e.,} 
\begin{equation}
	\mathbf{z}_M^{(i)}|\mathbf{x}_M^{(i)}\sim\mathcal{N}\left(\mathbf{\mu}_M^{(i)},\mathsf{diag}(\mathbf{\sigma}_M^{(i)})\right),\,M\in\left\{O,A\right\},\,i=1,\cdots,N
\end{equation}
where $\mathbf{\mu}_M^{(i)}\in\mathbb{R}^d$ is the mean vector, $\mathsf{diag}(\cdot)$ diagonalizes the variance vector $\mathbf{\sigma}_M^{(i)}\succ\mathbf{0}\in\mathbb{R}^d$ to form the co-variance matrix. Thereupon, to characterize $\mathbf{z}_M^{(i)}$, it only requires to learn the distributional parameters $\mathbf{\mu}_M^{(i)}$ and $\mathbf{\sigma}_M^{(i)}$. For this goal, we employ two \highlight{ lightweight shallow extractors}, \highlight{denoted as} $\mathsf{Le}_1\left(\cdot;\mathbf{\theta}_1^M\right),\,\mathsf{Le}_2\left(\cdot;\mathbf{\theta}_2^M\right)$ and parameterized with $\mathbf{\theta}_1^M,\,\mathbf{\theta}_2^M$, to deliver the mean and variance:
\begin{equation}
	\mathbf{\mu}_M^{(i)}=\mathsf{Le}_1\left(\mathbf{x}_M^{(i)};\mathbf{\theta}_1^M\right),\,\log\left(\mathbf{\sigma}_M^{(i)}\right)=\mathsf{Le}_2\left(\mathbf{x}_M^{(i)};\mathbf{\theta}_2^M\right)
\end{equation}
in which we define the output of $\mathsf{Le}_2\left(\cdot;\mathbf{\theta}_2^M\right)$ to be the logarithm of $\mathbf{\sigma}_M^{(i)}$ to ensure the positive definiteness of co-variance matrix.
\end{CJK}


